P-Reverb: Perceptual Characterization of Early and Late Reflections for Auditory Displays

We introduce a novel, perceptually derived metric (P-Reverb) that relates the just-noticeable difference (JND) of the early sound field(also called early reflections) to the late sound field (known as late reflections or reverberation). Early and late reflections are crucial components of the sound field and provide multiple perceptual cues for auditory displays. We conduct two extensive user evaluations that relate the JNDs of early reflections and late reverberation in terms of the mean-free path of the environment and present a novel P-Reverb metric. Our metric is used to estimate dynamic reverberation characteristics efficiently in terms of important parameters like reverberation time (RT60). We show the numerical accuracy of our P-Reverb metric in estimating RT60. Finally, we use our metric to design an interactive sound propagation algorithm and demonstrate its effectiveness on various benchmarks.

==> IEEE VR Atul Final 2019/Ack.tex <==
\section{Acknowledgments} The authors would like to thank the subjects who took part in
the user-study. This work was supported in part by ARO grant W911NF-18-1-0313, NSF grant 1840864, and Intel.


==> IEEE VR Atul Final 2019/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> IEEE VR Atul Final 2019/Section1.tex <==
\section{Introduction} 
Sound rendering uses auditory displays to communicate information to a user. \changes{Harnessing a user's sense of hearing enhances the user's experience and provides a natural and intuitive human-computer interface. Studies have shown a positive correlation  between the accuracy or fidelity of sound effects and the sense of presence or immersion in  virtual reality~\cite{larsson2002better,dubois2009engineering,rungta2016psychoacoustic}. Sound is also  an important cue for perceiving distance~\cite{zahorik2005auditory} and orientating oneself in an  environment~\cite{wilson2007swan}}. 

The sound emitted from a source and reaching the listener can be \changes{broken down into three components, described in more detail below: direct sound, early reflections, and late reflections or reverberation (Fig. \ref{fig:IR_image}). All three components of the sound field have perceptual relevance and have been extensively studied in psychoacoustics.  Direct sound gives us an estimate of the loudness and the distance to the sound source~\cite {zahorik2001loudness}.  Early reflections (ERs) arrive later than the direct sound, often in a range from $5$ to $80$ milliseconds.
Late reflections or reverberation (LRs) are generated when the sound signal undergoes a large number of reflections and then decays as it is absorbed by the objects in the scene.} 
%It degrades our sense of localization \cite{begault1992perceptual}, enhances auditory distance \cite{bronkhorst1999auditory}, g and reduces speech clarity \cite{payton1994intelligibility}.

Because of the importance of different components of sound fields, there has been considerable work on simulating these effects and incorporating them into auditory displays. %tend to incorporate these three components to varying degrees of accuracy. There is considerable work on simulating each of these components.  %each of these components  
Some of the commonly used methods 
approximate the sound field using artificial reverberation filters, which use 
%acoustic parameters such as
reverberation time $(RT_{60})$ to tune parametric digital filters~\cite{valimaki2012fifty}. These filters tend to have low computational requirements and are widely
%take only a few megabytes of space and a few milliseconds at runtime. As a result, they are widely
used for interactive auditory displays~\cite{kleiner1993auralization}. However, finding the right parameters for reverberation filters can be time-consuming and current methods do not provide sufficient fidelity. Geometric sound propagation methods work under the assumption that sound travels in straight lines and can be modeled using ray tracing~\cite{krokstad1968calculating}.
%, frustum tracing~\cite{chandak2008ad}, or beam tracing ~cite{funkhouser1998beam}. 
This allows resulting algorithms to model sound's interaction with the environment as it undergoes reflection and scattering.  Many techniques have been proposed to accelerate ray tracing, and current methods can generate early reflections (ERs) and late reflections (LRs) at  interactive rates  in dynamic scenes using high-order ray tracing (e.g., more than $100$ orders of reflections)~\cite{schissler2017interactive}. In practice, high-order ray tracing can be expensive and current interactive systems use multiple CPU cores on desktop workstations. The most accurate methods for sound rendering are based on wave-based acoustics, which  directly solve the acoustic wave equation using numerical methods.
%and can accurately simulate all sound effects, including low-frequency diffraction effects. 
However, their precomputation and storage overheads are very high and current methods are only practical for lower frequencies~\cite{mehra2012efficient,mehra2013wave,raghuvanshi2010precomputed}. 

Many applications, including games, virtual environments, and multi-modal interfaces require an interactive sound rendering capability, i.e., $20$fps or more. Furthermore, these systems are increasingly used on game consoles or mobile platforms where computational resources are limited. As a result, we need faster techniques to generate ERs and LRs in dynamic scenes for high-fidelity sound rendering. In particular, LR computation can be a major bottleneck.

%Overall, it remains a challenge to generate high-fidelity sound propagation
%There is considerable work on 

%As mentioned above, artificial reverberation filters see ubiquitous use in most auditory displays owing to their low computational and memory requirements. But tuning these filters requires the designers to \textit{guess} the reverberation parameters such as $RT_{60}$ based on their intuition, and this process can be time consuming for modeling the sound field in a perceptually correct way. Geometric methods, while accurate, require a high-end, multi-core desktop machine to accurately generate the sound field interactively. One can precompute the reverberation parameters by sampling the scene at multiple points and use a geometric acoustic system to estimate the parameters for use in reverberation filters, but running such a simulation (direct + early \& late reflections) requires high-order ray tracing and is thus expensive. Instead, we exploit a much cheaper alternative of precomputing reverberation parameters by only computing early reflections at the sample points. We then use a perceptually derived metric that relates the just-noticeable difference of early reflections and late reflections. This metric can then be used to \textit{estimate the regions where the reverberation parameters are likely to change in a perceptible way} allowing us to run the expensive, full simulation only at a select number of points.   


{\bf Main Results:} We present a novel, perceptually derived metric called $P-Reverb$ that relates the ERs to the LRs in the scene. Our approach is based on the relationship between the mean-free path ($\mu$) and reverberation (Eq. \ref{eqn:mfp}), and we use early reflections to numerically estimate the mean-free path of the environment. We conduct two extensive user evaluations that establish the just-noticeable difference (JND) of sound rendered using early reflections and late reflections in terms of the mean-free path. We derive our perceptually-based $P-Reverb$ metric by expressing the JNDs of early and late reflections in terms of the mean-free path. Moreover, our metric is used to \changes{efficiently} estimate the late reverberation parameter ($RT_{60}$). 
%in an interactive auditory display.
%ARE WE STILL TALKING ABOUT THIS PRECOPUTATION STEPWe use this metric to estimate regions in the scene where the \textit{late reverberation would vary within the JND based on the mean-free path computed using early reflections}. This significantly reduces the precomputation time to compute accurate reverberation parameters for a scene.
We have evaluated the accuracy of our perceptual metrics in terms of computing the mean-free paths and reverberation time and comparing their performance with prior algorithms based on analytic or high-order ray tracing formulations. The mean-free path is within $3\%$ and reverberation time is within $4.6\%$, which are within the JND values specified by ISO 3382-1~\cite{iso20093382}.  
% Moreover, we use our formulation to compute late reverberation for geometric sound propagation and improve the performance by 13-16X on complex models. 
Overall, we observe significant benefits using our $P-Reverb$ metric for fast evaluation of mean-free path and reverberation parameters for sound rendering and auditory displays. We have used for sound propagation and rendering in complex indoor scenes.
% RATHER TALK ABOUT INTERACTIVE SOUND RENDERING USING EARLY REFLECTIONS AND SPEEDUPS USING PRIOR METHODS.
% TALK ABOUT APPLICATIONS TO SIZE PERCEPTION.
% Overall, the novel components of our approach include:
 

% \begin{itemize}
% \item  A perceptually driven $ER-LR$ metric that  establishes the relationship between the JND of early reflections (ER) and late reverberation parameterized (LR) in terms of mean free paths. 
% 	\item An efficient precomputation method based on mean free paths to cluster similar reverberation regions into iso-reverb zones. Our metric accelerates this computation by an order of magnitude.
%     %Novel user-studies validating and establishing our precomputation metric
%     \item An efficient caching method to store and retrieve the early reflections based on spherical harmonics for interactive propagation. Moreover, we present a scheme to dynamically calibrate the reverberation filters at runtime.
% %    \item A speedup of 6x-10x at runtime compared to current geometric acoustics system
% %     \item Efficient modeling of energy transfer between iso-reverb zones.
% \end{itemize}

The rest of the paper is organized as follows. We give a brief overview of prior work in sound propagation and psychoacoustics in Section 2. We present our user evaluations establishing the $P-Reverb$ metric in Section 3. We provide validation results in Section 4 and describe our how our metric can be used in an interactive sound propagation system in Section 5.

% There is a considerable amount of work on simulating the interaction of sound within an environment as it undergoes reflections, scattering, and attenuation before reaching the listener. Many approaches have been developed to model sound propagation in virtual environments. At a broad level,  prior methods can be classified into artificial reverberation filters, geometric acoustics, and wave-based acoustics.

% Artificial reverberation filters use acoustic parameters such as reverberation time $(RT_{60})$, direct-to-reverberant ratio $(DRR)$, and  reverberation pre-delay to approximate sound propagation in an environment \cite{valimaki2012fifty}. These tend to have low computational requirements, taking only a few megabytes of space and a few milliseconds at runtime. They are widely used in game engines and VR systems and are usually designed by artists or game-audio designers for different regions of an environment.  This can be time consuming and the precomputed filters may not be able to accurately generate dynamic reverberation effects. Geometric propagation methods work under the assumption that sound travels in straight lines and can therefore be modeled using methods such as ray tracing \cite{krokstad1968calculating}, frustum tracing \cite{chandak2008ad}, or beam tracing \cite{funkhouser1998beam}. This allows geometric algorithms to model sound's interaction with the environment as it undergoes reflection and scattering.  Over the years, many acceleration techniques have been proposed to accelerate ray tracing, and current methods can generate early reflections (ER) and late reverberation (LR) at  interactive rates  in dynamic scenes using high-order ray tracing (e.g. more than $100$ orders of reflections)~\cite{schissler2017interactive}. In practice, high-order ray tracing can be expensive and current interactive systems use multiple CPU cores on desktop workstations. Wave-based acoustics directly solve the acoustic wave equation using numerical methods and can accurately simulate all sound effects, including low-frequency diffraction effects. However, their precomputation and storage overhead of these methods are very high and current methods are only practical for lower frequencies~\cite{mehra2013wave,raghuvanshi2010precomputed}.

%on the other hand, use the underlying mathematical formulation (acoustic wave equation) to accurately model all aspects of sound propagating through an environment. These methods tend to be very accurate, but their steep compute and memory requirements preclude their use in dynamic, interactive scene, although some precomputation-based methods have been used in static virtual environments  mehra2015wave}.  
% Current game engines and VR systems use either reverberation filters or precomputation-based  geometric approaches to generate sound effects at runtime~\cite{valimaki2012fifty,stavrakis2008topological,tsingos2009precomputing}. These methods have low computational overhead and can be easily integrated with the applications systems. However, they have many limitations.  The subdivision techniques used to partition the scene for geometric methods tend to be adhoc. The performance of reverberation filters varies as a function of the tuning parameters. Moreover, these methods cannot simulate dynamic reverberation effects, which are important for many  sound cues~\cite{zahorik2005auditory}.  

%In practice, their computational requirements are low 
%As virtual reality moves towards the mobile realm, the available compute and memory resources get more constrained, making the problem of modeling sound propagation on such devices increasingly challenging. Ray tracing based sound propagation \cite{schissler2014high}, while efficient on desktop machines, would require significant speed up in order to remain interactive on a mobile device. This is especially the case with indoor environments where reverberation is prominent, requiring 100s of bounces of specular and diffuse reflections. Artificial reverberation filters are well suited to the problem, but they are not physically accurate, especially when dealing with the non-diffuse part of the sound field. However, reverb filters can model the diffuse part of the sound field accurately provided the right parameters such as $RT_{60}$, $DRR$, etc.

%Given the goal of accurately modeling sound propagation on devices with limited resources, an obvious approach is to use reverb filters that have been tuned based on the parameters of the environment. A typical method of implementation in game engines is to manually specify a spherical or cubical "reverb-zones" that are supposed to have similar reverberation characteristics. This approach is based on the designer's sense of what constitutes a region of similar reverberation characteristics and may not account for the scene's geometry and materials. Another approach could be to precompute the sound propagation data using an offline, accurate geometric acoustic system for use at runtime without having to resort to ray-tracing. However, a naive approach to precomputation could result in it taking an inordinate amount of time and storing unnecessary data which would then have to be loaded onto the memory-constrained mobile device. A third approach could be using a downsampled ray-tracing method \cite{schissler2018interactive} that uses a very limited number of rays at runtime to estimate the acoustic parameters of the environment. But such an approach can get easily overwhelmed as the number of sources in the scene increases or if the scene complexity is too high. Our approach is based on the observation that reverb filters can model diffuse sound fields with good accuracy when provided with the correct parameters. A and limited to a physically-correct \textit{iso-reverb zone}, given that ray tracing can accurately compute these required parameters. We therefore use a state-of-the-art ray tracing based sound propagation system to efficiently precompute the parameters of our iso-reverb zones and also cache the early reflections for use at runtime. Our approach is designed with two main constraints in mind: minimizing precomputation time and efficiently caching the necessary propagation data to enable plausible reverberation at runtime for a high number of sources without resorting to ray-tracing.

% \noindent{\textbf{Main Results}}: We present a new approach for interactive sound propagation that exploits perceptual properties of sound fields in terms of reverberation characteristics. We use a precomputation based approach and present a novel scheme to subdivide the scene into {\em iso-reverb zones}. An iso-reverb zone corresponds to a region of a scene, where the reverberation time $(RT_{60})$ varies imperceptibly. We exploit this property of  an iso-reverb zone to generate the reverberation parameters efficiently, and those parameters are then used to dynamically calibrate the reverberation filters for high-fidelity sound rendering. Moreover, we present a new method for computing early reflections based on spherical harmonics and caching. Overall, our runtime approach has almost the same overhead as artificial reverberation filters, but the sound effects have auditory perceptions that are comparable to those in a high-order ray tracing based system.

% A key aspect of our approach is to designing and using a perceptual metric to precompute iso-reverb zones.  In order to precompute the iso-reverb zones, one would typically need to compute the late reverberation for a set of sample points in a scene and then cluster the points based on the JND of late reverberation parameters such as $RT_{60}$. However, precomputing $RT_{60}$ values for a set of sample points in a scene could be expensive because this parameter typically requires hundreds of orders of specular and diffuse reflections. In order to speedup our precomputation stage, we exploit the close relationship between the mean-free path and $RT_{60}$ \cite{joyce1975sabine} and note that the mean-free path can be approximated by only considering the specular reflections in the scene \cite{beranek2014mean}. We perform extensive user studies to establish a data-driven relationship ($ER-LR$ metric) between just-noticeable difference (JND) of early reflections and late reverberation in terms of the mean-free path of the environment.  
% %We then establish a perceptual relationship ($ER-LR$ metric) between early reflections and late reverberation in terms of the mean-free path that 
% We use this metric to estimate regions in the scene where the \textit{late reverberation would vary within the JND based on the mean-free path computed using early reflections}. This significantly reduces the precomputation time and we do not need to perform high-order ray tracing at runtime to compute LR. 
% % We uNEED TO EXPLAIN 
% % 1. WHY JND IS SUFFICIENT FOR PERCEPTUAL EVALUTION.
% % 2. WHY WE CHOOSE TO COMPUTE THE RELATIONSHIP BETWEEN EARLY ER, LR IN TERMS OF MEAN-FREE PATH. WHY DO YOU CHOOSE MEAN-FREE PATH. GIVE A REFERENCE FOR ITS PERCEPTUAL BENEFITS FOR SOUND EFFECTS?

% We have evaluated our algorithm for generating sound effects on complex scenes and can generate the sound effects for a large number of sound sources at $50-100$ fps on a desktop CPU using only two threads for sound propagation. We also compare the runtime performance and auditory perception with a state of the art interactive geometric propagation system~\cite{schissler2017interactive}. We observe up to 16$\times$ improvement in runtime frame rate with comparable auditory perception. 

==> IEEE VR Atul Final 2019/Section2.tex <==
\section{Background \& Related Work} 
In this section, we give an overview of prior work in sound propagation, psychoacoustic characteristics, and related areas.

\subsection{Reverberation}
Reverberation forms the late sound field and is generated by successive reflections as they diminish in intensity. Reverberation is regarded as a critical component of the sound field. Many acoustic parameters such as the reverberation time (RT60) and clarity index (C50 and C80) are used to characterize reverberation~\cite{kuttruff2016room}. 
%In particular, ($RT_{60}$) is widely used in different applications~\cite{skaalevik2010reverberation}. 


\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{images/IR.jpg}
\caption{We highlight the different components of the sound field. The sound directly reaching the listener is called the direct sound, the reflections that reach in the first $80$ ms are called early reflections (ERs), while the reflections following the early reflections that show a decaying exponential trend are called late reflections or reverberation (LRs). Our $P-Reverb$ metric presents a new perceptual relationship between ERs and LRs and we use it for fast sound rendering.}
 \vspace*{-0.1in}
\label{fig:IR_image}
\end{figure}


\subsubsection{Reverberation Time ($RT_{60}$):} $RT_{60}$ is defined as the time for the sound field to decay by $60$dB. A well-known expression used to compute the reverberation time is given by Sabine's formula, which gives the relationship between the RT60 of a room in terms of its volume, surface area, and the total absorption coefficients of the materials used: 
\begin{equation}
RT_{60} \approx 0.1611sm^{-1}\frac{V}{Sa},
\end{equation}
where V is the total volume of the room in $m^{3}$, S is total surface area in $m^{2}$, $a$ is the average absorption coefficient of the room surfaces, and $Sa$ is the total absorption in sabins. In this paper, we use $RT_{60}$ as the main reverberation parameter and use our $P-Reverb$ metric for fast computation in complex scenes.

\subsubsection{Mean-Free Path} The mean-free path (MFP) of a point in the environment is defined as the average distance a sound ray travels in  between collisions with the environment and is directly related to the $RT_{60}$ \cite{kuttruff2016room}:
\begin{equation}
RT_{60} = k\frac{\mu}{log(1 - \alpha)},
\end{equation}
where $k$ is the constant of proportionality, $\mu$ is the mean-free path, and $\alpha$ is the average surface absorption coefficient. A closed form expression ~\cite{bate1947mean} for computing the mean-free path is given by:
\begin{equation}
\mu = \frac{4V}{S},
\label{eqn:mfp}
\end{equation}
where $V$ is the volume of the environment and $S$ is the surface area. 
The mean-free path can be computed to a reasonable degree of accuracy by only considering the specular reflection paths in the scene \cite{vorlander2000room}. We use our $P-Reverb$ metric for fast computation of $\mu$ using only ER in complex scenes.

\subsection{Sound Propagation and Acoustic Modeling}
Artificial reverberators provide a simple mechanism to add reverberation to ``dry" audio, which has led to their widespread adoption in the music industry, virtual acoustics, computer games, and user interfaces. One widely used artificial reverberator was introduced by Schroeder~\cite{schroeder1961colorless} and it uses digital nested all-pass filters in combination with a parallel bank of comb filters to produce a series of decaying echoes. These filters require parameters such as reverberation time $(RT_{60})$ to tune the all-pass and comb filters. Geometric methods work on the underlying assumption of the rectilinear propagation of sound and use ray tracing to model the acoustics of the environment~\cite{krokstad1968calculating}. Other geometric methods include beam tracing~\cite{funkhouser1998beam} and frustum tracing~\cite{chandak2008ad}. In practice, ray tracing remains the most popular because of its relative simplicity and generality and because it can be accelerated on current multi-core processors. Over the years, research in ray tracing-based sound propagation has led to efficient methods to compute specular and diffuse reflections~\cite{schissler2014high} for a large number of sound sources~\cite{schissler2017interactive}.

\subsection{Early \& Late Reflections: Psychoacoustics}
Early reflections (ERs) have been shown to have a positive correlation with the perception of auditory spaciousness and are very important in concert halls. \cite{barron1971subjective,blauert1986auditory} showed that adding early reflections generated the effect of ``spatial impression'' in subjects. Early reflections are also known to improve speech clarity in rooms. \cite{bradley2003importance} showed that adding early reflections increased the signal-to-noise ratio and speech intelligibility scores for both impaired and non-impaired listeners. %\cite{arweiler2011influence} studied the effect of the spectral characteristics of early reflections on speech intelligibility and found that early reflections help but not as efficiently as the direct sound. 
\cite{hartmann1983localization} showed that early reflections that come from the same direction as the direct sound reinforce localization, while those coming from the lateral directions tend to de-localize  the sources. 

Late reflections or reverberation (LRs) provide many perceptual cues. Source localization ability deteriorates in reverberant conditions, with localization accuracy decreasing in a reflecting room compared to the same absorbing room~ \cite{hartmann1983localization}. Reverberation has a negative impact on speech clarity and ~\cite{knudsen1932architectural} showed the reduction in the number of sounds heard correctly in the presence of reverberation.
%\cite{galster2007effect} found that speech intelligibility decreases significantly in a small, highly reflective rooms. 
Although reverberation decreases localization accuracy and speech intelligibility, it is known to have positive effects with respect to the perceived distance to a sound source in the absence of vision~\cite{zahorik2005auditory}. 

While there is considerable work on  separately characterizing the perceptual effects of ERs or LRs, we are not aware of any work that establishes any relationship between ERs and LRs. $P-Reverb$ is a metric that establishes the relationship between the respective JNDs and uses them for interactive sound rendering.


\subsection{Estimating Reverberation Parameters} Given the importance of reverberation to the overall sound field, multiple methods have been established to measure the reverberation parameters over the years. $(RT_{60})$, in particular, is considered to be the most important parameter in estimating reverberation and has been referred as the `The mother of all room acoustic parameters' \cite{skaalevik2010reverberation}. The most commonly used method to estimate reverberation time was given by Schroeder, and uses a backward time integration approach. \cite{ratnam2003blind} presents a method for blind estimation of $RT_{60}$ that does not require previous knowledge of sound sources or room geometry by modeling reverberation as an exponentially damped Gaussian white noise process. \cite{lollmann2008estimation} describes a method to estimate reverberation time using maximum likelihood estimator from noisy observations. \cite{vorlander1994comparison} presents a comparison of different methods for estimating $RT_{60}$.




% \subsection{Precomputed Reverberation Parameters} 
% These algorithms try to reduce the runtime cost of generating sound effects either by precomputing the required acoustic parameters or subsampling the scene.
% %at runtime to estimate the parameters to tune an artificial reverberator. 
% These include techniques that reduce the runtime ray sampling budget  by using parametrized filters~\cite{schissler2018interactive}, though they still perform high-order ray-tracing. Other methods subdivide the scene using a cell-and-portal approach and precompute the energy transfer between each cell by computing a reverberation graph~\cite{stavrakis2008topological}. At runtime, they use this graph to construct a time-domain decay envelope for each sound source which feeds into an artificial reverberation engine.
% %that uses block based finite impulse response convolution to the input sound signals. 
% Tsingos~\cite{tsingos2009precomputing} uses a ray-tracer to precompute the image source gradients of the environment at user-provided key positions. At runtime, the image sources are interpolated from these key positions to the actual source position using the gradients. Our approach also precomputes the iso-reverb zones using our perceptual ER-LR metric, which offers many benefits. Compared to prior methods, we can generate dynamic reverberation effects at runtime without performing high-order ray tracing.


==> IEEE VR Atul Final 2019/Section3.tex <==


% \section{Acoustic Field \& Iso-Reverb Zones} In this section, we give an an overview of our sound propagation algorithm based on iso-reverb zones. 
% An environment's sound field is composed of three distinct parts~\cite{kuttruff2016room}:
% \begin{enumerate}
% \item Direct sound between source and listener,
% \item Early reflections (ER),
% \item Late reverberation (LR).
% \end{enumerate}
% While direct sound can be efficiently computed at runtime using a simple visibility checks, early reflections and late reverberation can be modeled using  multiple orders of ray bounces in a scene. ER correspond to the reflected sounds that reach the listener up until $80 - 100 ms$ after the direct sound. They help in  localization~\cite{hartmann1983localization} and convey spatial information about the environment~\cite{barron1981spatial}.  LR, on the other hand, forms the diffuse part of the sound field  and gives an impression of the size of the environment, level of furnishing and absorptivity~\cite{hodgson1991evidence}. However, computing dynamic LR can be relatively expensive because we need to perform high-order ray tracing.

% % MAKE IT CLEAR THAT YOUR ENVIRONMENT IS ASSUMED TO BE STATIC. MENTION THIS AS A LIMITATION AT THE END OF THE PAPER AS WELL.


% Our approach exploit the perceptual characteristics of the sound field. Our goal is to compute the appropriate characteristics as part of the precomputation stage, and use them at runtime to quickly compute ER and LR for given source and listener positions.
% %In order to avoid these expensive multiple ray bounces at runtime, it is important to come up with a way to cache data in the precomputation stage that can be retrieved efficiently at runtime and used to reconstruct the early reflections and late reverberation. 
% We exploit the diffuse characteristics of LR to find regions of spaces where the changes in reverberation are imperceptible to human hearing and then cluster them into \textit{iso-reverb zones} .  
% % Early reflections, on the other hand, are very heavily dependent on the relative source/listener positions and the scene geometry, and hence show a lot more variation. This makes it challenging to precompute them without having to store an inordinate amount of data. 
% Given these goals for precomputation and caching ER and LR, it is important to represent the associated data in a memory efficient manner. Our overall pipeline (Figure \ref{fig:rz_pipeline}) is divided into two distinct stages: precomputation to compute the iso-reverb zones and the associated parameters, and runtime system that uses these parameters to compute the reverberant sound effects by performing simple visibility checks and reverberation filters. Both these stages are optimized for computational and storage efficiency.

% \begin{figure*}[t]
%     \center
% 	\includegraphics[width=1\textwidth, height=5cm]{images/rz_pipeline.png}
% \caption{LABEL THE PRECOMPUTATION AND RUNTIME STAGES IN THE FIGURE: We highlight different stages of our  sound propagation and rendering pipeline. During the precomputation stage, we sample the scene at uniformly-spaced points and compute the early reflections.
% %instead of computing the full (late reverberation) simulation to speed up precomputation. 
% Based on our perceptual ER-LR metric, 
% %relating the JND of early reflections and late reverberation ($ER \Leftrightarrow LR$ metric), 
% we cluster the points into zones within the JND of late reverberation. At runtime we use a combination of the listener's location, the early reflection cache and the iso-reverb zone's parameters to calibrate a Schroeder-type filter and perform auralization dynamically.}
% \label{fig:rz_pipeline}
% \end{figure*}


% \subsection{Precomputation} 
% We begin our precomputation stage by uniformly sampling the 3D scene and generating a set of sample points $P$. where the spacing between each point depends on the scene volume. In our benchmarks, $|P|$ was on the order of $10^3 - 10^4$.  Furthermore, we assume that the propagation effects are computed for $f$ frequency bands. 

% \subsubsection{Early Reflection Cache} As mentioned above, early reflections (ER) form a crucial component of the sound field, giving us important spatial and localization cues about the environment and making it very important to incorporate them in the rendered sound. Unfortunately,  unlike LR, ER vary significantly with the relative source/listener positions and the scene geometry. This  makes it challenging to cache them during the precomputation stage them without storing a large amount amount of data. Our approach to caching ER involve creating a set of $n$ concentric spheres centered around the origin of the scene. For each point $ p \in P$, we compute the ER and record the intersection of the reflected rays with these concentric spheres. For each intersection, we store the energy of the ray hitting the sphere for each frequency band $f$ and the intersection point. Once the intersection points and the ray energy values for all $p$ are recorded, they are projected onto a compact spherical harmonic basis:    

% \begin{equation}
% E(\mathbf{y}, \omega) \approx  \sum_{l=0}^{l_{max}} \sum_{m=-l}^{l} Y_{l}^{m}(\textbf{y})c_{l}^{m}(\omega),
% \label{eq:SH}
% \end{equation}
% where $l_{max}$ is the order of the spherical harmonic, $c_{l}^{m}(\omega)$ are the vector of the basis harmonic coefficients as a function of frequency, $\omega$ is the center frequency for the band, $Y$ is the spherical harmonic basis, and $\mathbf{y}$ are the intersection points on a sphere. In total, for each point $p$, we save $(l_{max} + 1)^2 \times n \times \#freq$ values to represent the early reflections in the scene efficiently. These values can be retrieved easily at runtime, and using the cached spherical harmonic coefficients, we can approximate the energy due to the early reflections efficiently without having to store an explicit early reflection ray cache.

% \subsubsection{Late Reverberation Cache} LR constitutes the most computationally expensive part of computing the sound field and often requires hundreds of orders of diffuse reflections. This is especially pronounced in highly reverberant, indoor scenes where the sound could take a long time $(> 2 - 3 sec)$ to decay. Even with a state-of-the-art geometric ray tracer, computing the late reverberation is the slowest part of the simulation and can take around $5 - 10 \times$ more time than the  computation time  needed to compute direct sound and early reflections \cite{schissler2017interactive}. To capture the variation in reverberation parameters $(RT_{60})$, we would need to perform a dense sampling of the scene, which would be slow. 
% %Given the dense sampling of the scene that we need to do in order to capture the variation in reverberation parameters, computing the late reverberation for all the points would be too slow.

% Instead of computing the full sound field (direct + early reflections + late reverberation) at each point, $ p \in P$, we restrict our approach to only computing the early reflections (ER). Our choice is driven by the fact that although early reflections do not predict the late reverberation directly, they can be used to compute a parameter (mean-free path) that can, in turn, be used to predict late reverberation \cite{dalenback1996room}. The mean-free path (MFP) of a point in the environment is defined as the average distance a sound ray travels in  between collisions with the environment and is directly related to the $RT_{60}$ \cite{kuttruff2016room}:
% \begin{equation}
% RT_{60} = k\frac{\mu}{log(1 - \alpha)},
% \end{equation}
% where $k$ is the constant of proportionality, $\mu$ is the mean-free path, and $\alpha$ is the average surface absorption coefficient. A closed form expression for computing the mean-free path is known for simple shapes (sphere, cube, rectangle)~\cite{bate1947mean}:
% \begin{equation}
% \mu = \frac{4V}{S},
% \label{eqn:mfp}
% \end{equation}
% where $V$ is the volume of the environment and $S$ is the surface area. For arbitrary shapes, $\mu$ can be calculated numerically using Monte-Carlo integration techniques ~\cite{allred1958applications}. 

% The mean-free path can be computed to a reasonable degree of accuracy by only considering the specular reflection paths in the scene \cite{vorlander2000room}, and we exploit this property. We compute the mean-free path at a point $p$ while computing the early reflections during our precomputation stage and storing them. Fig. \ref{fig:MFP} shows the distribution of the mean free path at the sample points in a cathedral scene computed using the early reflections. The next step in this stage is to use the perceptual relationship (ER-LR) between the early reflections (characterized by $\mu$) and the actual $RT_{60}$. This  enables us to classify different points as having imperceptible reverberation characteristics, thus allowing us to create the iso-reverb zones without having to perform expensive late reverberation computation during our precomputation stage.  The perceptual metric (ER-LR) establishes the relationship between the just-noticeable difference for the early reflections $(JND_{er})$ and the just-noticeable difference for late reverberation $(JND_{lr})$ in terms of the mean-free path $(\mu)$ of the sample points $p$ in the environment. In the next two sections we describe our user evaluation, which enables us to formalize the relationship of the $ER-LR$ metric in terms of the mean-free path.

% \begin{figure}[h]
% 	\includegraphics[width=0.99\columnwidth]{images/cathedral_MFP.png}
% \caption{The mean-free path values at the sample points $P$ for the Sibenik Cathedral. Notice how changes in the local shape of the cathedral cause the MFP values to change, indicating that the reverberation parameters would also change at these points. In this scene, $|P|$ was around 3K.}
% \label{fig:MFP}
% \end{figure}
\section{Perceptual Evaluations and P-Reverb} In this section, we describe two user evaluations that establish the just-noticeable difference (JND) for early and late reflections in terms of the mean-free path. Further, we show the relationship between the two JND values, thereby establishing our $P-Reverb$ metric. 

\subsection{Experiment I - Just-noticeable difference of ERs}
In this experiment, we seek to establish the just-noticeable difference $(JND_{er})$ of sound rendered using only direct and early reflections. In Experiment II, we establish the relationship between $JND_{er}$ and sound rendered using the full simulation (direct + early + late reverberation) $JND_{lr}$. 

\paragraph{Participants:} 106 participants took part in this web-based, online study. The subjects were recruited using a crowd-sourcing service. All subjects were either native English speakers or had professional proficiency in the language.

\paragraph{Apparatus:} The online survey was set up in Qualtrics. The impulse responses were generated using an in-house, realtime, geometric sound propagation engine written in C++, while the convolutions to generate the final sounds were computed using MATLAB.

\paragraph{Stimuli:} \changes{The stimuli were sound clips derived from $7$ cube-shaped rooms with increasing edge lengths such that their MFPs (Eq. \ref{eqn:mfp}) varied from $2 - 2.2$m in increments of $0.033$m. The range of lengths was chosen with the experimental goal in mind, namely, to extract a psychophysical function showing a gradient in perceived sound similarity relative to edge-length difference.  The walls of the rooms had reflectivity similar to that of an everyday room. The source was a sound of clapping, which was chosen because it represents a broadband signal.} The clips were filtered in 4 logarithmically spaced frequency bands ($0 - 176$Hz, $176 - 775$Hz, $775 - 3408$Hz, and $3408 - 22050$Hz) to evaluate the effects of frequency on $JND_{er}$. Each of these $4$ filtered clapping sounds was convolved with the early impulse responses of the $7$ rooms. The final sound clip was around $4$ seconds long and contained $3$ distinct parts: $1.5$ seconds of the clapping sound in Room 1 ($\mu = 2m$), $1$ second of silence, and another $1.5$ seconds of clapping in a second room drawn from $1 - 7$ ($\mu = [2 to 2.2]m$). \changes{All sounds were recorded assuming that the listener and the source were located at the origin $(0,0,0)$. Given this symmetry, the sounds were rendered in mono with both speakers playing the same sound.} 

\paragraph{Design \& Procedure:} \changes{To estimate the JND, our experiment used the method of constant stimuli~\cite{gescheider2013psychophysics} with a within-subject design. A stimulus comprised a sound clip containing Room 1 and one of the 7 possible comparison rooms (including Room 1). For each clip the subjects heard, they were asked to identify if the first clapping sound seemed to be different from the second clapping sound by selecting yes or no. Note this is a similarity judgment, not a discrimination.  A block of judgments consisted of $28$ clips ($4$ frequencies x $7$ comparison rooms paired with Room 1). A block was repeated $5$ times, giving a total of $140$ clips (4 frequencies x 7 possible rooms paired with Room 1 x 5 blocks). The ordering of the clips was randomized within a block. Each subject judged all $140$ stimuli.  Before starting the experiments, subjects listened to a sample clip for familiarization. The subjects were required to have a pair of ear-buds/headphones to take part in the study, which took an average of $25$ minutes to complete.}

\paragraph{Results \& Analysis:}  Fig. \ref{fig:MFP_JND} shows the proportion of responses in which rooms were judged as sounding different, over all participants, as a function of the comparison level of $\mu$. The first data point corresponds to rooms that were objectively identical, providing a baseline.  The data essentially increases linearly with a larger $\mu$, showing greater discrimination up to Room $6$ ($\mu = 2.17$), after which ($\mu = 2.2$) the discriminatory ability seems to taper off. The standard errors are low and consistent, indicating the robustness of the results. 

An interesting observation is the near-invariance of subjects' ability to discriminate across the frequency bands. This was verified by an ANOVA analysis with factors of edge length (or $\mu$) and frequency. The analysis showed significant main effects for both factors of edge length $F(6, 180) = 61.78, p < 0.05, \eta^{2}_{p} = 0.673 $ and frequency $F(3, 90) = 2.95, p = 0.037, \eta^{2}_{p} = 0.09 $. The interaction between edge length and frequency was also significant $F(18, 540) = 1.66, p = 0.04, \eta^{2}_{p} = 0.052 $, reflecting that the performance decrement at the largest edge length is slightly greater for frequency band $4$.  However, the $\eta^{2}_{p}$ values are very low for effects involving frequency. Thus, while the effects of frequency show statistical significance, they are small in effect size and do not reflect consistent variation in frequency across edge length (or $\mu$).  Therefore, for the purposes of constructing an overall rule, using data averaged over the  frequencies is  a valid simplification, particularly if the largest value of edge length is excluded. Fig. \ref{fig:MFP_JND_AVG} shows the results averaged over the frequency for Rooms $1 - 6$. As shown in the figure, the data fits a linear function well, with $R^{2} = 0.98$.  
Given our linear fit:
\begin{equation}
\delta = 3.89\mu - 7.5
\label{eq:linear_jnd_fit},
\end{equation}
we can easily estimate the $JND_{er}$ by considering the MFP values ($\mu_{JND}$) where the subjects successfully discriminated the sounds 50\% of the time given by $\mu_{JND} = \mu_{50\%} - \mu_{room1} = 2.06 - 2 = 0.06 m$. This tells us that a change in $\mu$ greater than 0.06m would result in perceptually differentiable sounds when using \textit{early impulse responses}, but it doesn't necessarily indicate if the relationship holds if the sounds were rendered using the \textit{full impulse response} (LR). This led us to conduct the next experiment to establish the relationship between the JND of early reflections $(JND_{er})$ and the JND of full impulse response or late reverberation $(JND_{lr})$.

\begin{figure}[h]
	\includegraphics[width=0.99\columnwidth]{images/MFP_JND.png}
\caption{The psychometric function for sound rendered using the early reflections for the 4 frequency bands. The Y-axis shows the proportion of responses indicating the sounds were different. \changes{We see a clear, linear trend between increasing $\mu$ and the probability of responding different, until the last room $\mu = 2.2$, where the responses seem to flatten out. }}
\label{fig:MFP_JND}
\end{figure}

\begin{figure}[t]
	\includegraphics[width=0.95\columnwidth]{images/avg_mfp_jnd.png}
\caption{The average JND over the frequency bands. The Y-axis shows the proportion of responses indicating that a difference was \changes{judged. The psychophysical function is essentially linear, showing that the probability of judging the sounds as different increases linearly with the increasing mean-free paths of the rooms. }}
\label{fig:MFP_JND_AVG}
\end{figure}

\subsection{Experiment II - Relationship between $JND_{er}$ \& $JND_{lr}$} 
Once we have established the perceptibility threshold or $JND_{er}$ of ERs, we need to relate this to the $JND_{lr}$ of LRs. Our goal is to use these relationships to cluster points $p \in P$ with similar reverberation characteristics. We conducted another user study based on the results of the first study, described above. 

\paragraph{Participants} $31$ participants took part in this online, web-based study. The subjects were recruited using the same crowd-sourcing service as in the previous experiment. All subjects were either native English speakers or had professional proficiency in the language.

\paragraph{Apparatus} The apparatus was the same as in Experiment I. The full impulse responses were generated using our in-house, realtime, geometric sound propagation engine written in C++, with the convolutions being computed using MATLAB.


\paragraph{Stimuli} The sound source used was the same as in the previous experiment, filtered for the same logarithmically-spaced frequency bands. Given our goal of establishing the relationship between $JND_{er}$ and $JND_{lr}$, we use our previously computed psychometric  function (Eq. \ref{eq:linear_jnd_fit}), to compute the \textit{$6 \mu$ values corresponding to detection rates ranging from $0.2$ to $0.7$}. This gives us $6$ $\mu$ values that can then be used to compute the cube rooms' edge lengths using Eq. \ref{eqn:mfp}. These $6$ rooms and Room $1$ from the previous experiment serve as the environments in which the full impulse responses are computed. The material properties of the rooms were the same as in the previous experiment. Each sound clip in this case was about $6$ seconds because of the increased length of full impulse response, with $2.5$ seconds of clapping in Room $1$, followed by a second of silence, followed by $2.5$ seconds of clapping in Rooms $2 - 7$. The total number of sound clips was $14$0, as before ($4$ frequency bands x $7$ rooms x $5$ blocks). The ordering of the sound clips was randomized within each block.

\paragraph{Design \& Procedure} The study design was the same as in the ER study. Before starting the study, the subjects were asked to listen to a sample sound clip from the $28$ clips computed above for familiarization. The source and listener locations in the rooms were located at $(0,0,0)$. The sound was rendered in mono. The subjects took an average of $30$ minutes to complete the study. 


\begin{figure}[h]
	\includegraphics[width=0.95\columnwidth]{images/JND_RT_60.png}
\caption{The psychometric function for sound rendered using the full impulse response $(LR)$ for the $4$ frequency bands. The Y-axis shows the proportion of responses indicating sounds were judged to be different. In this case, we observe more variability for the different frequency bands, which could be attributed to the greater sensitivity of human hearing to a more accurate signal (compared to the less accurate ER signal). Overall, however, the responses can be modeled as a linear function with reasonable accuracy.}
\label{fig:JND_RT_60}
\vspace*{-0.15in}
\end{figure}

\paragraph{Results \& Analysis} Fig. \ref{fig:JND_RT_60} \changes{shows the proportion of responses judging the sounds as different, as a function of increasing $\mu$ or edge-length}. As before, we performed an ANOVA to assess the effect of edge length and frequency. The analysis showed significant main effects for edge length $F(6, 180) = 61.78, p < 0.05, \eta^{2}_{p} = 0.673 $ and frequency $F(3, 90) = 2.95, p = 0.037, \eta^{2}_{p} = 0.09 $. The interaction between edge length and frequency was also significant $F(18, 540) = 1.66, p = 0.04, \eta^{2}_{p} = 0.052 $. Again, the effect size for terms involving frequency was low, allowing us to average the responses for the frequency bands. Fig. \ref{fig:JND_RT60_AVG} shows the values averaged for the $4$ frequency bands.
    


\begin{figure}[h]
	\includegraphics[width=0.95\columnwidth]{images/JND_RT60_AVG.png}

\caption{The average JND over the frequency bands for the full impulse response signal. \changes{The Y-axis shows the proportion of responses indicating a judgment of difference}. The psychophysical function is not as linear as the early reflection signal, but a linear function approximates the subject responses reasonably well ($R^2 = 0.87$), accounting for most of the variability.}
\label{fig:JND_RT60_AVG}
% \vspace*{-0.15in}
\end{figure}



\subsection{$P-Reverb$ Metric} Fig. \ref{fig:RT60_VS_MFP} shows the relationship between the sounds rendered using only the early responses and the sounds rendered using the full impulse response. Note that the first point for both functions corresponds to two identical stimuli, and no difference is expected.  However, beginning at the smallest edge lengths where objectively different stimuli were presented, the figure shows that the subjects were more likely to \changes{differentiate} between sounds rendered with the full impulse response than they were with sounds rendered using only the early reflections. A difference in \changes{difference judgments is expected,} because the  full impulse response conveys more information about the space and is supposed to enable better perceptual differentiation than the early impulse response, thus giving a lower JND for the full impulse response, i.e., $JND_{lr} < JND_{er}$ .

To establish a mathematical relationship between the two JNDs, we consider the ratio of the mean-free paths in both cases. The resulting figure is shown in Fig. \ref{fig:MFP_ADJ}. The linear fits are almost coincident after adding a constant offset of $0.02$, i.e. 
\begin{equation}
\frac{\mu_{JND_{lr}}}{\mu_{1}} + 0.02 = \frac{\mu_{JND_{er}}}{\mu_{1}},
\end{equation}
which gives a simple relationship between the two JND values:

\begin{equation}
\mu_{JND_{lr}} = \mu_{JND_{er}} - 0.02 \mu_{1},
\label{eq:jnd_rel}
\end{equation}
where $\mu_{1}$ is the mean-free path in Room $1$ = $2$m. Hence $\mu_{JND_{lr}} = \mu_{JND_{er}}- 0.04$ is the simple mathematical relationship or $P-Reverb$ for the JND values of the two signals. Given $\mu_{JND_{er}} = 0.06 m$ as derived above, we can easily compute the value of $\mu_{JND_{lr}}$ as being $0.02m$ for a reference room (Room 1) $\mu = 2m$, \textit{giving us the percentage change ($\frac{\mu_{JND_{er}}}{\mu_{Room 1}} = 1 \%$) in the mean-free path values that constitute the JND for late reverberation}, when using early reflections.

It turns out that  Eq. \ref{eq:jnd_rel} can be interpreted as a ``first-order" approximation to a function that expresses the mathematical relationship between two multi-dimensional perceptual phenomena that are dependent on frequency, edge length, method of rendering, material parameters, etc. However, any function that accounted for the small frequency dependencies in the observed psychometric data and accommodated the effects of more complex environments and material parameters would have to be substantially more complicated than the linear relationship that we derive here. The value of the present formulation lies in its reasonable approximation of the observed effects with only one derived parameter. 

We would also like to note that, although psychometric functions are usually fitted using sigmoid functions, our design did not require us to do so. A sigmoid function approach would have been suitable had we started with a value somewhere in the middle and taken a range of values above and below. This would have yielded two end-cases with the non-standard stimulus being judged smaller 100 \% of the time; similarly, the larger non-standard stimulus would be judged as such 100 \% of the time. In our approach, however, we never tested anything smaller than the standard, which led us to values that rose to the ceiling. Consequently, a linear fit to this function accounted for most of the variance $(93 \%)$. A better fit could be achieved using a quadratic fit (accounting for $99 \%$ of the variance), but at the expense of adding a parameter. A sigmoid function, too, would add another parameter without yielding much gain. Therefore given the fact that our linear fit accounts for most of the variability, we chose to not use a sigmoid fit. 

% We would like to note that a function not neglecting the minor frequency dependencies in the observed psychometric function and considering the effects of more complicated environments and material parameters would be significantly more complicated than what we see here and as such, Eq. \ref{eq:jnd_rel}, should be interpreted as a `first-order' approximation function establishing the mathematical relationship between two, multi-dimensional perceptual phenomena. We use this first-order approximation in our pipeline to  cluster the points into iso-reverb zones. 





\begin{figure}[h]
	\includegraphics[width=0.95\columnwidth]{images/RT_60_vs_MFP.png}

\caption{This plot shows the overlaid psychometric functions for signals
rendered using the early reflections (blue) and full impulse response (orange). Note that the first data point corresponds to differences being reported when the stimuli are objectively identical.  Although the full impulse data shows a greater departure from a linear relationship beyond that point, the results are similar to the early reflection function, offset by a constant, allowing us to establish a simple, linear relationship between $JND_{er}$ and $JND_{lr}$ in terms of the mean-free path.}
\label{fig:RT60_VS_MFP}
% \vspace*{-0.15in}
\end{figure}


\begin{figure}[h]
	\includegraphics[width=1\columnwidth]{images/MFP_ADJ.png}

\caption{The psychometric function with a constant offset adjustment. We consider the ratio of the mean-free path for the different rooms to the mean-free path of Room 1. The resulting linear fits for the two cases (early reflections and full impulse response) coincide once a constant offset of 0.02 is added to the ratio for the full impulse response. This highlights the accuracy of our model.}
\label{fig:MFP_ADJ}
\end{figure}

% \subsubsection{Iso-Reverb Zone} Once we have computed the $JND_{er}$ of our early reflection signal and established its relationship to the JND of the full impulse response signal ($JND_{lr}$), we can use it for our precomputation algorithm. Our algorithm is used to cluster the points $p \in P$ that would generate regions with similar reverberation characteristics. There are multiple ways in which the clustering can be performed. We use agglomerative clustering \cite{defays1977efficient} with a single linkage as our choice of clustering method. The distance measure was Euclidean and the threshold was set using our previously established psychometric relationship (Eq. \ref{eq:jnd_rel}).

% Since the number of clusters is not known a priori, we use the elbow method \cite{thorndike1953belongs} to determine the number. We use this method to generate regions of similar reverberation (Fig. \ref{fig:CLUSTER}). For each iso-reverb zone computed by our algorithm, we run the full simulation \textit{once} per zone and associate the reverberation time $RT_{60}$ to all the sample points belonging to that zone. 

% \begin{figure}[t]
% 	\includegraphics[width=0.95\columnwidth]{images/cathedral_MFP.png}

% \caption{The clustering of the mean-free path values for the Cathedral scene. The regions that show variation within the JND limits as established by our $ER \Leftrightarrow LR$ are grouped into a single iso-reverb zone. (Placeholder image) FINISH THIS }
% \label{fig:CLUSTER}
% \end{figure}



==> IEEE VR Atul Final 2019/Section4.tex <==
\section{Results \& Evaluation}
% In this section, we showcase the accuracy of the $P-Reverb$ metric in predicting the $RT_{60}$ values on different benchmarks. 
Our approach consists of two primary numerical steps: computing the mean-free path $(\mu)$ using early reflections (ERs), and predicting $RT_{60}$ using our perceptually established $P-Reverb$ metric. We first validate the use of early reflections (ERs) to compute the mean-free path ($\mu$) in various environments. Next, we highlight the validation of the $P-Reverb$ metric in terms of its accuracy in predicting $RT_{60}$. 
% In particular, we compare the values computed using $P-Reverb$ metric with prior numerical or high-order ray racing methods (i.e. the ground truth).


% \begin{figure}[t]
% 	\includegraphics[width=\columnwidth]{images/rzteaser.jpg}
% \caption{Complex benchmarks used to evaluate the performance of our modified sound propagation algorithms. Instead of performing high-order ray tracing, we use the $P-Reverb$ metric to compute the reverberation parameters and acoustic effects. This  improves the performance of overall sound rendering by $13-16$X over prior propagation algorithms~\cite{schissler2014high}}.
% \label{benchmars}
% \vspace*{-0.15in}
% \end{figure}

 

% \subsection{Validation} We evaluate the accuracy  of our  $P-Reverb$ metric. 


\begin{figure*}[h]
    \center
	\includegraphics[width=1\textwidth]{images/preverbvalidation.png}
\caption{ We highlight the application of $P-Reverb$ metric to predict variations in $RT_{60}$ in a scene composed of interconnected rooms of different shapes and volumes: (a) shows the variation in $\mu$ along a path that goes through three rooms with volumes 135 $m^3$, 256$m^3$, and 125 $m^3$ from left to right; (b) shows three regions $(1,2,3)$ along the path roughly corresponding to the three rooms, where $\mu$ changes within the JND specified by the $P-Reverb$ metric. This indicates that the reverberation in these regions would vary imperceptibly, as is indicated by the uniformity of the $\mu$ values; (c) shows rapidly varying $\mu$ values as one approaches the apertures between the connected rooms, indicating that $RT_{60}$ would also vary rapidly. This is expected because the geometry varies rapidly in these regions and validates the accuracy of our perceptual metric $P-Reverb$.}

\label{fig:preverbvalidation}
\end{figure*}

\subsection{Mean-Free Path Computation} Our $P-Reverb$ metric depends on the numerically computed mean-free values that are computed using early reflections. The mean-free path is the average distance a sound ray would travel between collisions and we use ERs to estimate this distance. As mentioned, Eq. (\ref{eqn:mfp}) can be used to compute mean-free path values in terms of the volume ($V$) and surface area ($S$).  Table \ref{table:MFP_Validation} highlights the accuracy of our computed mean-free path values ($\mu_{er}$) as compared to the analytical values given by Eq. \ref{eqn:mfp}. We use $500$ rays and 20 bounces for each ray to compute our $\mu_{er}$ value as:
\begin{equation}
\mu_{er} = \frac{\sum d_{i}}{n \times b},
\end{equation}
where $d_{i}$ is the distance traveled by a sound ray on the $i^{th}$ bounce, $n$ is the total number of rays, and $b$ is number of bounces per ray.


{\small
\begin{table}[h]
%         \centering
        % \small
        \begin{tabular}{|r|c|c|c|c|c}
        \hline
      {$\mathbf{Shape}$} & {$\mathbf{Dim. (m)}$} & {$\mathbf{\mu_{er} (m)} $} & {$\mathbf{\mu_{an} (m)}$} & {$\mathbf{\% error}$}  \\
        \hline
        
        Cube              &   5                       & 3.3    & 3.33 & 1\\      
        Rect. Prism       &   (2,3,4)                 & 1.87   & 1.85 & 1.3\\
        Sq. Pyramid       &   (2.8, 3) (b, h)         & 1.16   & 1.18 & 1.7\\
        Room with Pillars &   (5,6,12)                & 3.14   & 3.04 & 3\\
%
        \hline
        \end{tabular}
        \vspace*{0.1in}
\caption{\textbf{Mean-free path Computation:} We show the accuracy of computing $\mu_{er}$ using early reflections for differently shaped rooms. The closed-form expression in Eq \ref{eqn:mfp} gives us the analytical value for the mean-free paths in each of the rooms $\mu_{an}$. We observe that ERs can closely approximate the analytically obtained $\mu_{an}$. The Room with Pillars  is shown in Fig. \ref{fig:roomwithpillars}. Even for a scene with multiple obstacles, our method computes the mean-free path while inducing a maximum error of only $3\%$. }
\label{table:MFP_Validation}
% \vspace*{-0.15in}
\end{table}
}

\subsection{$RT_{60}$ using $P-Reverb$ Computation} The $P-Reverb$ metric predicts regions in a scene where the late reverberation is likely to vary imperceptibly. Conversely, it can estimate regions where the late reverberation would vary in a perceptually noticeable manner. We demonstrate the effectiveness of the $P-Reverb$ metric in finding regions of similar reverberation characteristics by considering a scene shown in Fig. \ref{fig:preverbvalidation}. The scene is composed of different interconnected rooms of varying shapes and volumes. Since reverberation is a function of the volume and shape of the room, it is likely to vary as one moves from one room to another. We consider a path that traverses three different connected rooms and compute the mean-free path along the path using  ERs. Fig. \ref{fig:preverbvalidation}(a) shows the variation in $\mu$ as we move along the path.  We group the regions along the path where $\mu$ varies within the JND threshold computed using our $P-Reverb$ metric (as shown in Fig. \ref{fig:preverbvalidation}(b)), as Regions $1$, $2$, and $3$. Based on the $P-Reverb$ metric, each such region is likely to have an imperceptible sound in terms of $RT_{60}$. We illustrate this in Table \ref{table:preverbvalidationtable}. The $\mu_{mean}$ corresponds to the average mean-free path value for the entire region and $Diff._{max}^{\mu}$ corresponds to the maximum difference from the $\mu_{mean}$ for all the points in that region (i.e., a measure of variance). The $RT_{60}^{mean}$ represents the average value of the reverberation times for the region, while $Diff._{max}^{RT_{60}}$ corresponds to the maximum difference from $RT_{60}^{mean}$. For regions where $\mu$ varies within the JND specified by the $P-Reverb$ metric, the $RT_{60}$ values vary within 5\% of the $RT_{60}^{mean}$. This is within established JND values for $RT_{60}$, as specified in ISO 3382-1 \cite{iso20093382} and correspond to imperceptible changes in late reverberation.

Fig. \ref{fig:preverbvalidation}(c) shows rapidly varying $\mu$ values, as one moves from one room to another. This indicates that the reverberation or $RT_{60}$ would vary rapidly in these regions. Since none of these values falls within the JND specified by $P-Reverb$, they cannot be grouped to create regions where reverberation would be imperceptible. This is expected because coupling of spaces is known to affect the sound energy flow and the change of $RT_{60}$ close to the coupling aperture \cite{jing2008visualizations}.



{\small
\begin{table}[t]
%         \centering
        % \small
        \begin{tabular}{|r|c|c|c|c|c}
        \hline
      {$\mathbf{Region}$} & {$\mathbf{\mu_{mean} (m)}$} &  {$\mathbf{Diff._{max}^{\mu}}$}  & {$\mathbf{RT_{60}^{mean} (s)}$} & {$\mathbf{Diff._{max}^{RT_{60}}}$} \\
        \hline
        
        1 &   2.45  & 1.1 \%  & 0.65 & 4.6 \% \\      
        2 &   3.64  & 0.5 \% & 1.27 & 2.4  \% \\
        3 &   3.11  & 1.1 \%  & 1.03 & 3.6 \% \\
%
        \hline
        \end{tabular}
        
\caption{\textbf{Mean-Free Path and Reverberation Time Computation:} We show the average values computed using high-order ray tracing for the three different regions shown  in Fig.  \ref{fig:preverbvalidation} and the differences from the average values. Each of these rooms corresponds to imperceptible regions based on our $P-Reverb$ metric. The numerical value shows a maximum variation of $5\%$, which is within JND values of $RT_{60}$. The exact $RT_{60}$ was computed using high-order ray tracing with $300$ bounces. }
\label{table:preverbvalidationtable}
% \vspace*{-0.15in}
\end{table}
}


\begin{figure}[t]
	\includegraphics[width=0.9\columnwidth]{images/roomwithpillars.png}

\caption{Room with Pillars: We illustrate the room with $8$ pillars and use this benchmark to estimate the effectiveness of our mean-free path computation in complex environments with obstacles. We observe less than $3\%$ error using our early reflection based method.}
\label{fig:roomwithpillars}
\vspace*{-0.1in}
\end{figure}

% \subsubsection{Perceptual Validation}
% In this experiment, we evaluated the perceptual validity of our $P-Reverb$ metric in estimating the $RT_{60}$ metric. We use a state-of-the-art geometric ray tracer based on \cite{schissler2014high} as our control and a system that uses a Schroeder-type artificial reverberation filter to render the test sound. The artificial filter is tuned using parameter computed using our $P-Reverb$ metric. 

% \paragraph{Participants} X participants took part in this web-based, on-line study.   The subjects were recruited using a crowd-sourcing service.  All subjects were either native English speakers or hadprofessional proficiency in the language.

% \paragraph{Apparatus} The sounds rendered using the two systems (geometric and filter-based) were recorded directly as wav files sampled at 44.1 kHz.
% \paragraph{Stimuli} The stimuli consisted of 3 cube-shaped rooms $(R_{1}, R_{2}, R_{3})$ with increasing volumes ranging from [x-y] $m^{3}$.  The walls of the rooms, again, had reflectivity similar to that of an everyday room. The source was the same as before which is the sound of clapping filtered in the same 4 logarithmically spaced frequency bands. The source was rendered using the two methods under consideration $(M_{1}, M_{2})$, where $M_{1}$ is the full-fledged geometric acoustic system, and $M_{2}$ is the sound rendered using the artificial reverberation system using the $P-Reverb$ metric. Therefore, each stimulus is defined as a combination of room and methods, i.e., $(R_{i}, M_{j})$.

% \paragraph{Design \& Procedure} The experiment was a within-subject design, and each subject experienced all the sound clips. All sounds were recorded with the listener and source placed at the origin $(0,0,0)$. Before starting the experiment, the subjects were played a sample clip to familiarize them with the sound clips. The sounds were rendered in mono with both speakers playing the same sound. The subjects were required to have a pair of ear-buds/headphones to take part in the study. 

% \paragraph{Results \& Analysis}







==> IEEE VR Atul Final 2019/Section5.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1\textwidth]{images/clusteredPointsPReverb.jpg}
\caption{The figure shows how the $P-Reverb$ metric can be used to estimate regions where $RT_{60}$ would vary imperceptibly in a scene. The left figure shows a typical listener path in a scene. At each point along this path, we compute the mean-free path $\mu$ using the early reflection based method described. Then using the $P-Reverb$ metric, we cluster the points based on the $JND$ to give us clusters along the path where $RT_{60}$ would vary imperceptibly as shown in the right figure. }
% \vspace*{-0.15in}
\label{fig:clustering}
\end{figure*}





\section{Interactive Sound Propagation}  
In this section we describe how the $P-Reverb$ metric can be used for interactive sound propagation. As described in Sections 1. \& 2., the sound reaching the listener from a source has three components: direct sound, early reflections, and late reverberation as shown in Fig. \ref{fig:IR_image}. Geometric sound propagation algorithms use methods such as ray tracing to compute the ERs and LRs in the scene. Although early reflections can be computed cheaply, late reverberation computation remains a major bottleneck as it requires very high-order ray bounces in the scene for accuracy making these methods resource heavy. This prevents the use of these methods in interactive environments such as games, which tend to use cheap filter-based approaches (digital reverberation filters) to simulate late reverberation. Reverberation filters require parameters such as $RT_{60}$ to approximate late reverberation in an environment. One way in which reverberation filters can be parameterized accurately is to precompute the $RT_{60}$s along the listener's path in the scene using a high-fidelity geometric sound propagation algorithm such as \cite{schissler2014high}, and then use these precomputed $RT_{60}$ values at runtime in the filter. This would avoid costly high-order ray tracing to simulate reverberation at runtime, but can incur a high precomputation cost requiring us to run high-order ray tracing for every point along the listener's path. We now describe how using our $P-Reverb$ metric can reduce the precomputation cost of computing $RT_{60}$ values in the scene. 




% \subsection{Geometric Sound Propagation}

\subsection{Sound Propagation using $P-Reverb$} 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{images/filter.jpg}
\vspace*{-0.15in}
\caption{The figure shows the schematic of a typical Schroeder-type filter used in our implementation. The input is processed through a parallel bank of comb filters that create the delayed version of the input signal. The output of this parallel bank goes through a series connection of allpass filters. These filters require parameters like $RT_{60}$ to approximate the late reverberation in a scene.}

\label{fig:filter}
\end{figure}

\subsubsection{Precomputation} We  use our $P-Reverb$ metric to accelerate the pre-computation of late reverberation for an interactive sound propagation system using a Schroeder-type reverb filter to simulate late reverberation (Fig \ref{fig:filter}).  We sample a given scene at multiple points along the listener's path and use a geometric sound propagation method ~\cite{schissler2014high} to compute early reflections by placing an omni-directional sound source tracing $20$ orders of specular reflections at each of these points. Next, using Eq. \ref{eqn:mfp} we compute the mean-free paths at each of these points. Using the $P-Reverb$ metric, we clusters points on the path where $\mu$ varies within its JND, indicating that these regions will have perceptibly similar $RT_{60}$ values (Fig. \ref{fig:clustering}). Finally, using \cite{schissler2014high}, we compute the $RT_{60}$ values once for each computed region using high-order (300 bounces) reflections to get a high quality estimate. Table \ref{table:precomp_tab} shows the speed-up obtained using the $P-Reverb$ metric in precomputation stage. The results were obtained on a multi-core desktop using single thread for the computations.  


\subsubsection{Runtime} At runtime, the direct sound computation is done through visibility testing; if a source is visible to the listener, its distance to the listener is used to attenuate the sound pressure according to the inverse distance law. The late reverberation computation is performed using the precomputed $RT_{60}$ values in the previous stage. Given the listener position, a look-up is performed to ascertain the cluster (precomputed in the previous step) the listener position belongs to. Since, an $RT_{60}$ value is associated with each cluster, this is now used as a parameter into the reverberation filter. As long as the listener in within this cluster, $P-Reverb$ metric tells us that $RT_{60}$ value would vary imperceptibly.    
The accompanying video shows the performance of our metric on three different scenes.

\subsection{Benchmarks}

\paragraph{Sun Temple} This scene consists of spatially varying reverberation effects. As the listener moves throughout the scene, the reverberation characteristics vary from being almost dry in the semi-outdoor part of the temple to being reverberant in the inner sanctum. 

\paragraph{Shooter Game} This scene showcases the ability of our method to handle very large scenes. It shows an archetypal video game with multiple levels. As the listener moves from part of the scene to another, it shows our method's ability to handle highly varying, large, virtual environments. 

\paragraph{Tuscany} This scene has two different structures, a house and a cathedral, separated by an outdoor garden. The two structures have very different reverberant characteristics owing to their different geometries, and as the listener moves from the house to the cathedral going through the outdoor garden, the reverberant varies accordingly.  

{\small
\begin{table}[t]
        \centering
        \small
        \begin{tabular}{|r|c|c|c|c|c|c|c}
        \hline
      {$\mathbf{Scene}$} & {$\mathbf{\#Vert.}$} & {$\mathbf{\#P}$} &  {$\mathbf{T_{ER}(ms)}$} &{$\mathbf{T_{LR} (ms)}$} & {$\mathbf{\#P}$}   & {$\mathbf{Speed-up}$} \\
        \hline
        
        Sun Temple      &   215k   &   2301   & 40.2 & 124.2 &  53  & 3x\\
        Tuscany      &   135k   &   1945   &   47.5 & 150.7 & 110   & 3x\\
        Shooter Game      &   49k   &   3235   &  16.7 & 68.4 & 43    & 4x\\
%
        \hline
        \end{tabular}
        \vspace*{0.1in}
\caption{\textbf{Precomputation Performance Analysis:} We highlight the speed-up in precomputation stage  using the $P-Reverb$ metric. $\#P$ is the number of points along the listener path, $T_{ER}$ is the avg. time taken at each point using ERs,$T_{LR}$ is the average time taken at each point using LRs, and $\#P$ is the number of clusters found using our $P-Reverb$ metric.}
\label{table:precomp_tab}
% \vspace*{-0.08in}
\end{table}
}

% At runtime, the direct sound computation is performed using a single visibility checking operation for each source in the scene. If a source is visible to a listener, the distance to the source is used to attenuate the source's sound pressure value. The late reverberation is added to the scene by retrieving the $RT_{60}$ value precomputed in the previous step and feeding that to a Schroeder-type artificial reverberation filter \cite{schroeder1961colorless}. Since late reverberation computation forms the most expensive step in the computation of a sound field, we get a significant speed-up in the runtime performance by avoiding expensive high-order ray tracing which would otherwise be required to get the $RT_{60}$ values (Table \ref{table:runtime_tab}).

% {\small
% \begin{table}[h]
%         \centering
%         % \small
%         \begin{tabular}{|r|c|c|c|c|c|}
%         \hline
%       {$\mathbf{Scene}$} & {$\mathbf{Our Method (ms)}$} & {$\mathbf{Ray-Tracing(s)}$} & {$\mathbf{Speed-up}$} \\
%         \hline
        
%         Maze             &   4 & 52 & 13x\\      
%         Cathedral        &   6 & 96   & 16x\\
%         House            &   4 & 57   & 14x\\
% %
%         \hline
%         \end{tabular}
% \caption{\textbf{Runtime Performance Analysis:} We highlight the runtime performance of our system. As the table shows, we get a speedup of 13-16x in our benchmarks. }
% \label{table:runtime_tab}
% % \vspace*{0.25in}
% \end{table}
% }

% In this section, we describe our interactive sound propagation algorithm, which uses the precomputed iso-reverb zones described above.  As described in Section 3, the sound field is composed of the direct sound, early reflections, and late reverberation. Out of these, we have already described the precomputation of the early reflections and late reverberation parameters. The direct sound does not need to be cached and can be easily computed based on the visibility of the source to the listener. To retrieve the early reflection cache and the reverberation parameters, the first step requires us to establish the nearest sample point $p$, which is an index to the ER cache and the iso-reverb zone.

% \subsubsection{Direct Sound} The direct sound computation is performed using a single visibility checking operation for each source in the scene. If a source is visible to a listener, the distance to the source is used to attenuate the source's sound pressure value. Once the nearest sample point $p$ to the source position is found, we lookup its spherical harmonic coefficients stored in the ER cache for $p$. This is performed using a simple ray cast that samples the two concentric spheres closest to the listener at nine points for each sphere. Fig. \ref{fig:ER_RETR} shows a case where the listener is in between the blue and the green sphere with cones of rays cast in the forward and backward directions to compute the intersection points with the spheres. These intersection points are then converted into their spherical coordinates and, along with the spherical harmonic coefficients computed in the precomputation stage, give us cached early reflection values on both spheres using Eq. \ref{eq:SH}. The early reflection values at the listener are then obtained by linearly interpolating along the corresponding forward and backward rays.

% \subsubsection{Late Reverberation} Once the direct sound and gain factor are computed, the last step consists of finding the iso-reverb zones for the source to compute the late reverberation parameters. This is done by retrieving the precomputed $RT_{60}$ parameter associated with the iso-reverb zone to which the point $p$ belongs. The precomputed $RT_{60}$ is used as one of the parameters to tune the all-pass and comb filters. The direct-to-reverberant ratio is established using the following expression of this relationship \cite{schissler2018interactive}:
% \begin{equation}
% g(\omega) = \sqrt[]{\frac{I^{total}_{\omega}}{I^{total}_{reverb,\omega}}},
% \end{equation}
% where $g(\omega)$ is frequency-dependent gain factor of the filter, $I^{total}_{\omega}$ is the total intensity of the IR, and $I^{total}_{reverb,\omega} = \frac{RT_{60}}{6ln10}$. We use the combination of $RT_{60}, DRR$, and reverberation pre-delay to tune the all-pass and comb filters of our artificial reverberator to produce the desired reverberation effect. 

==> IEEE VR Atul Final 2019/Section6.tex <==
\section{Conclusion, Limitations and Future Work}

 We present a novel perceptual metric that highlights the relationship between the JNDs of early reflections and late reverberation. Our metric is based on two user studies and can be used for fast computation of mean-free-paths and reverberation time in complex environments without high-order ray tracing. Our metric can be used to predict regions in an environment where the reverberation time is likely to vary within its JND value. We evaluate the accuracy of these perceptual metrics and find their accuracy within $5\%$ of the actual values on our benchmarks. 
%  Furthermore, evaluated these metrics for interactive sound rendering and size estimation in virtual environments and 
 
Our approach has some limitations. Our $P-Reverb$ metric computation may not work in totally open environments since the mean-free path computation depends on the presence of collisions with the obstacles in the scene.  Our $P-Reverb$ metric can be regarded as an approximation to a complex function that corresponds to a multi-dimensional perceptual phenomenon dependent on source frequency, scene dimensions, method of sound rendering, material parameters, etc. As a result, we need to perform more evaluations that take other parameters into account. While we observe high accuracy in our current benchmarks, the accuracy could vary in more complex scenes.  Further, our metric tends to be conservative and overestimates the number of regions with similar $RT_{60}$ resulting in running more full simulations than optimal. That being said, it still \changes{significantly reduces the number of full simulations as shown in Table \ref{table:precomp_tab}}. \changes{Our experimental work also has limitations, including the restricted range of room sizes (motivated by the psychophysical goal), the fixed listener, and the restriction to mono rendering.} As part of future work, we would like to overcome these limitations and further evaluate our approach on complex scenes and use them for multi-modal rendering.


==> IEEE VR Atul Final 2019/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

